T-Lease: A Trusted Lease Primitive for Distributed Systems

A lease is an important primitive for building distributed protocols, and it is ubiquitously employed in distributed systems. However, the scope of the classic lease abstraction is restricted to the trusted computing infrastructure. Unfortunately, this important primitive cannot be employed in the untrusted computing infrastructure because the trusted execution environments (TEEs) do not provide a trusted time source. In the untrusted environment, an adversary can easily manipulate the system clock to violate the correctness properties of lease-based systems. We tackle this problem by introducing trusted lease -- a lease that maintains its correctness properties even in the presence of a clock-manipulating attacker. To achieve these properties, we follow a "trust but verify" approach for an untrusted timer, and transform it into a trusted timing primitive by leveraging two hardware-assisted ISA extensions (Intel TSX and SGX) available in commodity CPUs. We provide a design and implementation of trusted lease in a system called T-Lease -- the first trusted lease system that achieves high security, performance, and precision. For the application developers, T-Lease exposes an easy-to-use generic APIs that facilitate its usage to build a wide range of distributed protocols.

==> 2_background.tex <==
% -*- root: main.tex -*-
%!TEX root = main.tex

\section{Background}
\label{sec:background}

% \comment{Goals:
% \begin{itemize}
%     \item If the reader is a distributed systems researcher, he may not be familiar with SGX. Give background on TEEs, SGX, and the SGX features that we use. Also, explain TMP.
% \end{itemize}
% }

\subsection{Trusted Execution Environments and Intel SGX}

The global migration to cloud computing poses significant challenges to ensure secure operation of software systems.
Traditional approaches rely on hardware virtualization techniques~\cite{neiger_intel_2006, amdv_reference_manual} to isolate cloud tenants from each other, and on application-specific solutions to protect individual services.
However, the complexity of modern cloud stacks~\cite{openstack_org, opennebula_org, azure_stack, vsphere} makes ensuring security of the hypervisor problematic, as the extreme amount of code involved in VM management and orchestration virtually guarantees presence of bugs~\cite{wojtczuk_subverting_2008, wojtczuk_adventures_2008, weisse2018foreshadowNG}.
This undermines security even in those applications that have correct application-level defences implemented:
An attacker capable of subverting the hypervisor can directly read the application memory.
The same attack vector is available to malicious insiders on the cloud operator's side.

As a response to this threat, researches have developed a concept of Trusted Execution Environment (TEE).
An application running in a TEE is isolated from the control of privileged software and, thus, it becomes possible to build systems that are secure even if the OS or hypervisor is compromised.
The examples of TEE technologies are ARM TrustZone~\cite{trustzone}, AMD Secure Encrypted Virtualization~\cite{SEV}, and Intel Software Guard Extensions~\cite{SGXrelease}.

Intel SGX is the Intel's trusted execution technology that provides an \emph{enclave} primitive---an isolated region of memory containing code and data.
Any attempts to read from or write into the enclave memory from outside are forbidden on the hardware level, as well as code fetches from the enclave to outside.
The physical memory that backs the enclave is transparently encrypted using Memory Encryption Engine (MEE). Intel SGX provides a remote attestation mechanism~\cite{johnson2016intel} that allows remote users to verify that the software is indeed running inside SGX enclave on a genuine Intel CPU.

SGX guarantees confidentiality and integrity of data stored inside the enclave, as well as integrity of computations inside the enclave. As the host operating system still makes all resource management decisions, SGX cannot provide the availability.
% SGX offers no protection against several classes of microarchitectural attacks of both side-channel and Meltdown~\cite{Lipp2018meltdown}/Spectre~\cite{Kocher2018spectre} type.

To operate in the complex environment of general-purpose operating systems and complex x86 hardware, Intel SGX requires several service data structures: Secure Enclave Control Structure (SECS) and Thread Control Structure (TCS). SECS maintains information that concerns enclave as a whole, for example, enclave measurement, enclave memory base address, and enclave size. TCS contains information that is specific to a single thread, such as the location of State Save Area (SSA), which is used for storing register file during exceptions, and initial program counter value inside the enclave.

One important feature of SGX is its Asynchronous Enclave Exit (AEX) procedure. This procedure is triggered when a CPU exception or an interrupt is delivered to the core that is executing enclave code. It comprises the following steps:
\begin{itemize}
\item The register state and additional metadata are saved in the SSA.
\item The CPU state at enclave entry time is restored, with program counter pointing to the AEX handler instead of the original PC.
\item The CPU leaves the enclave mode, moving to unshielded user mode and then to kernel mode, where the exception is handled.
\end{itemize}

After handling the exception, the kernel executes the \code{IRET} instruction, which transfers control to the AEX handler. The AEX handler is supposed to return control to the enclave by executing an \code{ERESUME} instruction.

In our work, we rely on SCONE~\cite{scone2016}. SCONE is a trusted execution framework for execution of POSIX applications inside Intel SGX enclaves. As such, SCONE handles several problems that commonly arise: provides a POSIX environment (memory management and system calls) to the application, improves performance by using asynchronous system calls.
% SCONE is available on docker hub and includes a cross-compiler that supports to run
%most applications inside of enclave by simple recompilation.

SCONE supports remote attestation as well as the secure configuration of applications with the help of the SCONE Configuration and Attestation Service (CAS). In a nutshell, enclave application should use standard TLS with client and server authentication, whereas SCONE CAS distributes the TLS certificates in such a way that only attested applications can get access to their certificates.

\subsection{Timestamp Counter}

The x86 CPU architecture typically provides one of the following time sources: Time Stamp Counter (TSC) and High Precision Event Timer (HPET). TSC is the standard built-in clock available on the x86 architecture. It has low access latency (the latency of \rdtsc{} instruction is 12-20 cycles), and high resolution, which is accurate up to a cycle \cite{sdm}. Tick rate of TSC is independent of core power-saving modes and core frequency. The x86 architecture exposes two core-local MSRs that control the TSC value, for setting the TSC offset and the TSC value directly. Additionally, on the virtualized platforms, the x86 architecture exposes a VMCS field for setting a TSC tick rate. On modern hardware and operating systems, TSC is used as the default time source.

\subsection{Trusted Platform Module}
\input{2_tpm}

\section{Threat Model}
\label{sec:threat}

We consider an attacker that has full control over privileged software, such as host operating system and hypervisor. Thus, the attacker can manipulate offsets and rates of all timers where the rates can be manipulated. To achieve its goals, the attacker can also read and write to arbitrary memory locations where the hardware does not forbid this.

We assume that the CPU, including its SGX features, operates according to the specification. We also assume that in the normal operation mode, clocks have negligible drift rate. Another source of changes to the clock drift rate could be a physical attack: An attacker may cool down or heat up a discrete TPM or a motherboard reference frequency generator. We consider such attacks against TPM to be out of scope. Changes to the motherboard reference frequency are detected using TCS frequency check.
% \wo{shouldn't we exclude physical attacks? e.g., the crystal frequency depends on the temperature, hence dTPM time could be altered by cooling/warming the chip, though...}

Given this threat model, we provide a low latency timer that allows detecting a lower bound on the passed time in the presence of manipulations.

% \wo{I am not sure if this sentence should be a part of the threat model section. It describes system properties and not the security conditions it is designed to work in}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> Makefile <==
SHELL := /bin/sh

FILE := main
PUBLISH_FILE := $(FILE)-publish

texfiles := $(wildcard *.tex)
tables := $(wildcard tables/*.tex)
listings := $(wildcard listings/*.tex)
figures := $(wildcard figs/*.pdf)
styles := $(wildcard *.sty)

all_files = $(texfiles) $(tables) $(listings) $(figures) $(styles) refs.bib

to_pdf := pdflatex -synctex=1 -interaction=nonstopmode
pdf_publish := ps2pdf14 -dFastWebView=true -dPDFSETTINGS=/prepress

BIBTEX := bibtex

.PHONY: clean


# == Targets ==

all: $(FILE).pdf

$(FILE).pdf: $(FILE).tex $(all_files)
	@printf "Fist build...\n"
	@$(to_pdf) $(FILE)
	@printf "\n\nReferences...\n"
	@$(BIBTEX) $(FILE) || true
	@printf "\nSecond build...\n"
	@$(to_pdf) $(FILE)
	@$(to_pdf) $(FILE)
ifdef PUBLISH
	$(pdf_publish) $(FILE).pdf $(PUBLISH_FILE).pdf
endif

debug: to_pdf := pdflatex
debug: $(FILE).pdf

ieee_test:
	pdffonts $(PUBLISH_FILE).pdf
	pdfinfo $(PUBLISH_FILE).pdf	

clean:
	rm -f *.aux *.blg *.out *.bbl *.log *.soc *.synctex.gz $(FILE).pdf


==> listings/aex-detection.tex <==
% -*- root: ../main.tex -*-
%!TEX root = ../main.tex
\begin{figure}[t]
\begin{lstlisting}
<had_interrupt> :=
  if (SSA.PC == 0) {
    return false;
  } else {
    SSA.PC = 0;
    return true;
  }
\end{lstlisting}
\caption{Interrupt detection mechanism.}
\label{fig:aex-detection}
\end{figure}


==> listings/estimation.tex <==
% -*- root: ../main.tex -*-
%!TEX root = ../main.tex
\begin{figure}[t]
\begin{lstlisting}
int interrupt = <had_interrupt>;
current = rdtsc();
interrupt |= <had_interrupt>;
<check_results>

<check_results> :=
  if (no interrupt) {
    time += current - previous;
    previous = current;
  } else {
    <recover from the interrupt>
  }
\end{lstlisting}
\caption{Algorithm of interval estimation.}
\label{fig:estimation-algo}
\end{figure}


==> listings/spec-liveness.tex <==
% -*- root: ../main.tex -*-
%!TEX root = ../main.tex
\begin{figure}[tp]
\begin{lstlisting}[escapeinside={(*}{*)}, mathescape=true]
(*\textcolor{specGray}{\textbf{HolderAsksForLeaseGranterGrantsLease}}*) (*\equalDelta*)(*\label{line:s_p1}*)
($\exists$ m $\in$ msgs: m.msgType $\in${"ReqLease"} $\wedge$ (MaxNow-now)
$\geq$ MsgDeliveryMaxDelay $\wedge$ gEpochTimer > (MaxNow-now))
 $\leadsto$  ( gLeaseGranted $\neq$ {} )(*\label{line:e_p1}*)

(*\textcolor{specGray}{\textbf{GranterGrantsLeaseHolderHasValidLease}}*) (*\equalDelta*)(*\label{line:s_p2}*)
( $\exists$ h $\in$ LeaseHolders:  $\exists$ r $\in$ gLeaseGranted: r.lh = h
 $\wedge$  gExpireTimer = LeaseTime  $\wedge$ (MaxNow - now)$\geq$
  MsgDeliveryMaxDelay  $\wedge$ (lhEpochNumber[h]= 
  r.epochNumber) $\wedge$ lhEpochTimer[h]>(MaxNow - now)) 
  $\leadsto$ ($\exists$ h $\in$ LeaseHolders: lhState[h]={"validLease"})(*\label{line:e_p2}*)
\end{lstlisting} 
\caption{Liveness properties: holder eventually gets a lease.}
\label{fig:spec-liveness}
\end{figure}
% first; if a holder send a message to request a lease and we still have to time in the bounded time execution,, that we use, for the message to be processed by the granter (MaxNow-Now) >= MsgDeliveryMaxDelay and the granter will not be interrupted until the message is processed
% then by the end of MaxNow (eventually), the lease will be granted to some holder,, h= asked for if the lease if free or it will be already given to some one else so it is not free.

% second, if the granter grants the lease to some grantee (r.lh=h), and
% he sends a message directly (gExpireTimer = LeaseTime) and
% There is enough time for the message to reach (MaxNow- now) >= MsgDeliverMaxDelay and
% the responce is valid (grantee is not interrupted in betwee)
	% lhEpochNumber[h]= r.epochNumber
	% it will not be interrupted until the end of bounded time duration, (lhEpochTimer[h]>(MaxNow-now))
% then by the end of MaxNow, the holder will have the lease. (actually some holder will have it, it should be the same because of the safety ensurance, but it will be the same)


==> listings/spec-safety.tex <==
% -*- root: ../main.tex -*-
%!TEX root = ../main.tex
\begin{figure}[tp]
\begin{lstlisting}[escapeinside={(*}{*)}, mathescape=true]
(*\textcolor{specGray}{\textbf{ValidLease}}*) (*\equalDelta*)  $\forall$ h $\in$ LeaseHolders: (
 (lhState[h] = "validLease" $\wedge$ lhExpireTimer[h] $\neq$ 0)
  $\Rightarrow$  ( $\exists$ r $\in$ gLeaseGranted: r.lh = h ))
\end{lstlisting} 
\caption{Safety property: valid lease.}
\label{fig:spec-safety-validLease}
\end{figure}


==> listings/verification.tex <==
% -*- root: ../main.tex -*-
%!TEX root = ../main.tex
\begin{figure}[t]
\begin{lstlisting}
<recover from interrupt> :=
  previous = current;
  <check timer frequency>
  <application-specific recovery>

<check timer frequency> :=
  start_value = rdtsc();
  <constant-time operations>
  end_value = rdtsc();
  measurement = end_value - start_value;
  if (measurement < lower_threshold ||
      measurement > upper_threshold) {
    error();
  }
\end{lstlisting}
\caption{Interrupt recovery procedure.}
\label{fig:verification}
\end{figure}

